Photomeric analysis of eclipsing binaries: VY UMI, RU UMI AND GSC 04364-00648

We present the photometric analysis of \textit{BVR} and \textit{TESS} light curves of three eclipsing binaries (RU~UMi and purely studied VY~UMi, GSC 04364-00648), together with their period changes considering archival data and new minima times from our and \textit{TESS} observations. For the first time we detected wave-like variations with low-amplitude in $O-C$ residua of RU UMi, which can be interpreted as a consequence of the light-time effect caused by the 3rd invisible component with period 7370 days. Period increase with rate 2.56(9)$\times10^{-7}$~d/yr$^{-1}$ detected in the VY UMi system corresponds to mass transfer from the secondary to the primary component. For GSC 04364-00648 binary system we find some quadratic changes on the $O-C$ diagram, which corresponds to a period decrease with a high rate of $-2.26(5)\times10^{-5}$~d/yr$^{-1}$. We cannot assumptions about their nature, mainly due to short time of observation and uneven coverage of $O-C$ diagram. We also determined the absolute parameter of their components using the photometric solution and \textit{GAIA} distances.

==> README <==
-------------------------
THE REVMEXAA LATEX MACROS
-------------------------

Version: 3.26b (09 Feb 2015)

Author: William Henney (w.henney@crya.unam.mx)

Latest version available from:	http://www.crya.unam.mx/rmaa


USAGE
-----

This package is intended for the typesetting of papers that are being
submitted for publication in the main journal of the Revista Mexicana
de Astronomia y Astrofisica. The example document
rm-journal-example.tex serves both as simple documentation and as a
template for your own contribution.

Further details on the use of the macros are given in the "Guide for
Authors", authorguide.pdf


VERSION 3.2x RELEASE NOTES 
--------------------------

The main change in this release is a reorganization to give separate
packages for the Conference Series (rmsc3.2x.tar.gz or rmsc3.2x.zip)
and the main journal (rmaa3.2x.tar.gz or rmaa3.2x.zip).

The manuscript option for the main journal has been revamped and this
is now the default style, which should be used for all submissions.

A maximum of six keywords is now enforced. Exceeding this limit gives
a LaTeX compilation error.

There is also support for BibTeX, and a "review article" option has
been added to the main journal.

For more details, see the News section of http://www.crya.unam.mx/rmaa

DOWNLOAD AND INSTALLATION
-------------------------

The latest version of the macros can always be obtained from
|http://www.astrosmo.unam.mx/rmaa|. There are three different
packages, each designed for a different audience: authors of main
journal papers (e.g., |rmaa3.24.tar.gz|), authors of contributions to
conference proceedings (e.g., |rmsc3.24.tar.gz|), and editors of the
main journal or conference proceedings (e.g.,
|rmaa_editor3.24.tar.gz|). Please make sure you have the right
package. All packages are also provided in |.zip| format, chiefly for
the convenience of MS Windows users.

Once you have downloaded the relevant package archive file, move it to
the directory (folder) where you wish to work and unpack the
archive. The procedure to do this may vary between systems. From the
command line on Unix, Linux, or Mac OS X, you can use something like
|tar -zxf rmaa3.24.tar.gz|.

To test that everything is working, you should compile the example
document: |rm-journal-example.tex|. You will need to invoke |latex|
twice to get the cross references right. The procedure to view and
print the document will vary between systems. On Unix, Linux, or Mac
OS X, you can use |latex} and |dvips| to generate a postscript file
(which can be converted to PDF via |ps2pdf|), or alternatively you can
use |pdflatex| to generate a PDF file directly. Note that in the first
case, any included graphics must be in EPS format, while in the second
case, they must be in PDF, PNG, or JPG format. It is recommended that
you omit the file extension from the filenames in the
|\includegraphics| command, so that both |latex| and |pdflatex| can
automatically find the correct figure file.

Assuming that the example document compiled and printed correctly, you
can now start writing your own paper, using the example document as a
template. 


FILE MANIFEST for rmaaN.MM.tar:
-------------------------------

README			this file
rmaa.cls		LaTeX class file for typesetting RMAA articles 
rm-journal-example.tex	Example main journal paper and tutorial
authorguide.pdf		Guide for Authors 
example-fig.eps		Example of figure
example-badfig.eps	Example of how not to do a figure
example-fig.pdf		
example-badfig.pdf	
rmaa.bst		Bibtex style file (experimental)
GPL			Terms and conditions for copying, distribution
                        and modification


